Match the Script, Adapt if Multilingual: Analyzing the Effect of Multilingual Pretraining on Cross-lingual Transferability

Pretrained multilingual models enable zero-shot learning even for unseen languages, and that performance can be further improved via adaptation prior to finetuning. However, it is unclear how the number of pretraining languages influences a model's zero-shot learning for languages unseen during pretraining. To fill this gap, we ask the following research questions: (1) How does the number of pretraining languages influence zero-shot performance on unseen target languages? (2) Does the answer to that question change with model adaptation? (3) Do the findings for our first question change if the languages used for pretraining are all related? Our experiments on pretraining with related languages indicate that choosing a diverse set of languages is crucial. Without model adaptation, surprisingly, increasing the number of pretraining languages yields better results up to adding related languages, after which performance plateaus. In contrast, with model adaptation via continued pretraining, pretraining on a larger number of languages often gives further improvement, suggesting that model adaptation is crucial to exploit additional pretraining languages.

==> 2021_emnlp_multilingual_zeroshot/old_sections/40-results-back.tex <==
%\begin{table}[t!]
%\centering
%\small
%\setlength{\tabcolsep}{3pt}
%\begin{tabular}{lrrrrrr}
%\toprule
%\textbf{Pretrain} & \textsc{en} & \textsc{ru} & \textsc{zh} & \textsc{ar} & \textsc{hi} & \textbf{Unseen}  \\
%% Add indivdiual columns for each 5 language.
%\midrule
%\textsc{en}             & .950 & .243 & .155 & .119 & .087 & .193 \\
%Div-2 (+ru) & .952 & .766 & .163 & .128 & .058 & .210 \\
%Div-3 (+zh) & .951 & .785 & .272 & .124 & .084 & .213 \\
%Div-4 (+ar) & .950 & .777 & .273 & .510 & .070 & .258 \\
%Div-5 (+hi) & .949 & .732 & .287 & .471 & .521 & .256 \\
%\bottomrule
%
%\end{tabular}
%\caption{\label{tab:pos_unseen}
%\abr{pos} tagging accuracy after pretraining on a  diverse set of up to 5 languages and finetuning on English.
%The accuracy on unseen languages plateaued after 4 pretraining languages.
%}
%%\jbgcomment{Again, takeaway}
%\end{table}
%TODO: Confrim the results with different random starts/seeds


\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{\figfile{5morelangs_pos_acc}}
    \caption{
    \abr{pos} tagging accuracy after pretraining on a diverse set of up to 10 languages and finetuning on English.
    The accuracy improves until six languages on the given target languages.
    }
    \label{fig:pos_unseen_avg}
\end{figure}


\begin{figure*}[th]
    \centering
    \includegraphics[width=0.99\textwidth]{\figfile{pos_150K_accuracy}}
    \caption{
    \abr{pos} tagging accuracy on diverse pretraining languages (\textsc{en, ru, zh, ar, hi, es, el, fi, id, tr}) grouped by families of target languages, with Indo-European (\abr{ie}) languages further divided into subgroups following \abr{xtreme}.
    Points in the plot are more transparent if the languages are seen during pretraining and filled circles represent when the script type of the target languages are common with one of the pretraining languages.
    The accuracy gain is significant for seen languages, and also the languages from the same family and the same script type of the pretraining languages when added. 
    }
    \label{fig:pos_unseen}
\end{figure*}




%\section{Pretrained Models on Related Languages}
\section{Results}
\label{sec:results}

\jbgcomment{Don't like jumping directly from section into subsection}

We now show the experimental results to investigate  on each RQ.

\subsection{Findings for RQ1}
\label{sec:more_lang_better}
%Results on multiple tasks suggest that more languages are better for languages unseen during pretraining.

\paragraph{POS Tagging}
Figure~\ref{fig:pos_unseen_avg} shows the \abr{pos} tagging accuracy on the ten languages seen during pretraining and averaged over the 17 unseen languages.
%grouped by its language family following~\citet{hu20icml}.
On average, models pretrained on multiple languages have higher accuracy on unseen languages than the model pretrained exclusively on English, showing that the model benefits from a more diverse set of pretraining data. 
%\jbgcomment{avoid word ``perform''}
%The results in Table~\ref{tab:pos_unseen} further shows that the more languages the better for unseen languages during pretraining up to the five pretraining languages we experiment on.
However, the average accuracy only increases up to six languages. This indicates that our initial hypothesis "the more languages the better" might not be true. 
%The results in Table~\ref{tab:pos_unseen} further shows that the results improves up to four languages, and further.



%We see that the more pretraining languages are better for unseen languages, likely due to increasing the chance of target languages being related to one of the pretraining languages. 
%Figure~\ref{fig:pos_unseen} shows POS tagging results grouped by language families on both seen and unseen languages.
Figure~\ref{fig:pos_unseen} provides a more detailed picture, showing the accuracy for different number of pretraining languages for all seen and unseen target languages.
As expected, accuracy jumps when a language itself is added as a pretraining language. 
Furthermore, accuracy rises if a 
pretraining language from the same language family as a target language is added:
for example, the accuracy of Marathi goes up by $9.3\%$ after adding Hindi during pretraining, and the accuracy of Bulgarian increases by $31.2\%$ after adding Russian.
%, and the accuracy for \textsc{he} improves by $7.9\%$ after adding \abr{ar}.
This shows that related languages are indeed beneficial for transfer learning.
%, which supports the idea to just pretrain on as many languages as possible.
%There's also a consistent accuracy gain ($+3.7\%$) in the XNLI dataset too in Bulgarian, after adding Russian as the pretraining language (Table~\ref{tab:xnli_unseen})
Also, (partially) sharing the same script with a pretraining language (e.g., \abr{es} and \abr{et}, \abr{ar} and \abr{fa}) helps with zero-shot cross-lingual transfer even for languages which are not from the same family.
These results are consistent with the outcome of~\citet{muller2020when} and partially support the hypothesis by~\citet{pires2019multilingual} that shared scripts are effective on unseen languages.
%Finally, the results on unseen target languages from the same language family generally follow a similar trend, further supporting the claim by \citet{libovicky2020language} that multilingual models encode language-specific features.

Table~\ref{tab:pos_regression} shows the linear regression analysis results using typological features among target and pretraining languages.
For the script and family features, they are binary values set to one if a language with the same script or from the same family is included as one of the pretraining languages. 
For the family feature, we use the one from~\citet{xu2019crosslingual}.
For syntax and phonology features, we derive those vectors from URIEL database using lang2vec~\citep{littell2017uriel} following \citet{lauscher2020zero}.
We take the maximum cosine similarity between the target language and one of the all pretraining languages used.
Table~\ref{tab:pos_regression} further confirms that having a pretraining language which shares the same script contributes the most to positive cross-lingual transfer.

\begin{table}[t]
\centering
%\setlength{\tabcolsep}{7pt}
\small
\begin{tabular}{lrrc}
\toprule
\textbf{Features} & \textbf{Coef.} & \textbf{p-value} & \textbf{CI}\\
\midrule
Script            & \bf.061        & $<.001$          & [.050, .073]\\
Family            & .022           & $.004$           & [.007, .036]\\
Syntax            & .001           & $.905$           & [-.016, .018]\\
Phonology         & .021           & $<.001$          & [.009, .033]\\
\# pretrain langs & .011           & $.044$           & [.000, .022]\\
\bottomrule
\end{tabular}
\caption{\label{tab:pos_regression}
Regression analysis on the POS tagging accuracy with coefficients (Coef.), p-value, and $95\%$ confidence interval (CI). 
Large coefficient with a low p-value indicates that the feature significantly contributes to better cross-lingual transfer.
}
\end{table}



With the question of how many pretraining languages are optimal, we obtain mixed results. 
One consistent finding is that, for the large majority of languages, using only English yields the worst results for unseen languages. However, as also shown by the average in Figure~\ref{fig:pos_unseen_avg}, increasing pretraining language does not necessarily improve the accuracy. This indicates that, while we want more than one pretraining language, using a smaller number than the 100 commonly used pretraining languages is likely sufficient 
%and there is not need to add more pretraining languages 
unless we expect them to be closely related to one of the potential target languages. 
We further investigate it in Section~\ref{sec:xlmr}.

%However, the ``more languages the better'' trend is mixed for target languages which are not related to any of the five pretraining languages. There are languages (e.g., Greek, Vietnamese) drops when using 5 pretraining languages, however, some languages achieves highest accuracy by 5 pretraining languages (e.g., Farsi, Indonesian).

%In the next section, we further confirm the trend observed in this section also holds when adapting pretrained models to target languages.

\begin{table*}[th]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|rrrrr|rrrrrrrrrr}
\toprule
\textbf{Pretrain} & en & ru & zh & ar & hi & bg & de & el & es & fr & sw & th & tr & ur & vi \\
% Add indivdiual lumns for each 5 language.
\midrule
\textsc{en}           & .731 & .343 & .340 & .339 & .345 & .347 & .375 & .346 & .404 & .381 & .366 & .350 & .358 & .347 & .354 \\
Div-2        & .725 & .457 & .336 & .341 & .342 & .384 & .373 & .346 & .421 & .382 & .364 & .342 & .354 & .338 & .352 \\
Div-3     & .738 & .500 & .485 & .336 & .338 & .389 & .374 & .341 & .412 & .382 & .354 & .340 & .345 & .339 & .345 \\
Div-4    & .718 & .452 & .467 & .460 & .350 & .418 & .398 & .352 & .439 & .417 & .379 & .351 & .369 & .361 & .361 \\
Div-5    & .717 & .466 & .484 & .460 & .462 & .426 & .382 & .346 & .443 & .386 & .370 & .348 & .356 & .349 & .349\\
\bottomrule
\end{tabular}
\caption{\label{tab:xnli_unseen}
\abr{nli} accuracy on diverse pretraining languages over five seen (\textsc{en,ru,zh,ar,hi}) and 10 unseen languages.
More pretraining languages up to five are also generally better for unseen languages in the \abr{nli} task.
}
\end{table*}



\paragraph{NER}
Our \abr{ner} results show a similar trend, and therefore, only report the average (Figure~\ref{fig:ner_unseen_avg}) and full details are available in Appendix~\ref{sec:appendix_ner}.
For \abr{ner}, the transfer to unseen languages are more limited, likely due to small subset of tokens are labeled as entities when compared to \abr{pos} tags.

\begin{figure*}[th]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
        \includegraphics[width=0.45\textwidth]{\figfile{5morelangs_ner_f1}}
            \caption{
            \abr{pos} tagging accuracy of our models pretrained on diverse languages, \abr{xlm}-17, \abr{xlm}-100, and \abr{xlm-r} after finetuning on English.
            The models before adaptation are roughly on par regardless of the number of pretraining languages, and the models after adaptation is more affected by the related pretraining languages. 
            }
            \label{fig:pos_lowresource}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.45\textwidth]{\figfile{5morelangs_ner_f1}}
            \caption{
            \abr{pos} tagging accuracy of our models pretrained on diverse languages, \abr{xlm}-17, \abr{xlm}-100, and \abr{xlm-r} after finetuning on English.
            The models before adaptation are roughly on par regardless of the number of pretraining languages, and the models after adaptation is more affected by the related pretraining languages. 
            }
            \label{fig:pos_lowresource}
    \end{subfigure}
\end{figure*}


\paragraph{NLI}
Our \abr{nli} results show a similar trend  (Table~\ref{tab:xnli_unseen}): 
accuracy on unseen languages plateaus at relatively small number of pretraining languages. Specifically, Div-4 has the highest accuracy for 8 target languages, while Div-5 is best only for two target languages.
We again observe a gain in accuracy when adding related languages, such as an improvement of $+3.7\%$ accuracy for Bulgarian after adding Russian as a pretraining language.

%======================================================

%In this section, we further look into the research question explored in Section~\ref{sec:num_langs} from different point of view. 
%In this section, we further look into RQ1 ``the more pretraining languages the better?'' from different point of view. 
%We explore the effect of the number of languages with a fixed set of relatively diverse pretraining languages such as English, Russian, Chinese, Arabic, and Hindi.
%However, the question remains whether the number of languages that matters, or the selection of languages that matters more than the number of languages for languages unseen during pretraining.
%To investigate RQ1,  
%we select five related pretraining languages from Germanic family, namely English (\textsc{en}), Dutch (\textsc{nl}), German (\textsc{de}), Swedish (\textsc{sv}), and Danish (\textsc{da}).
%The relatedness between languages are measured by their pairwise cosine similarities of the binarized typological features from the URIEL database using lang2vec~\citep{littell-etal-2017-uriel}.


\subsection{Findings for RQ2}
\paragraph{POS Tagging } Figure~\ref{fig:pos_unseen_continued_el} shows the \abr{pos} tagging results for six languages after adaptation of the pretrained models via continued pretraining.
As expected, accuracy is overall higher than in Figure~\ref{fig:pos_unseen}.
%and the model with four, three, three, and three pretraining languages performs best for Greek, Vietnamese, Turkish, and French, respectively. 
%Importantly, Div-5 does not obtain the highest accuracy for \emph{any} language, even though this is the case for French and Greek without model adaptation. Furthermore, with the exception of Greek, the English-only model performs similarly to the best model. 
Importantly, 
%Div-10 obtains the highest accuracy for French and Farsi, where
there are accuracy gains in Farsi when adding Turkish ($+9.8\%$) and in Hebrew when adding Greek ($+7.7\%$), which are not observed before adapting models.
%Furthermore, with the exception of Greek, the English-only model performs similarly to the best model. 
We further investigate it in Section~\ref{sec:xlmr}.

%This gives support to our hypothesis that, with model adaptation, pretraining on more than one language is less likely to result in gains and more likely to hurt performance, since necessary language-specific knowledge can be acquired during continued pretraining.

\paragraph{NER} 
Figure~\ref{fig:ner_unseen_continued} shows the results on the \abr{ner} task.
There are similarities between \abr{pos} tagging in the improvement of \abr{bg} after adding \abr{ru}.
However, for example, there's limited improvement on \abr{fa} even after adding \abr{ar} regardless of partially shared scripts between the two languages.
This indicates that the effect of adding related pretraining languages is task-dependent. 

\paragraph{NLI} 
%Table~\ref{tab:xnli_continued} shows the results of all adapted models on XNLI. 
%Like our findings for \abr{pos} tagging, Div-5 does not generally perform best: only for one target languages (Turkish).
For \abr{nli}, we see a small increase in accuracy after adding a second pretraining language. 
%After that, improvements from adding additional languages is inconsistent across target languages: Div-2 is best for Vietnamese, while Div-4 is best for Greek and French. 
%However, 
Results for two to five pretraining languages are similar for all target languages and, for Greek and Turkish, still similar to the English-only model. This indicates that, similar to our findings for \abr{pos} tagging, a few pretraining languages could be sufficient for model adaptation. 
Full results are available in Appendix~\ref{sec:appendix_nli}.
Finally, our \abr{nli} results are low overall.
This is likely due to the size of the pretraining corpus is one of the top correlated feature for \abr{nli}~\citep{lauscher2020zero} unlike \abr{pos} tagging~\citep{hu20icml}.
%This is likely due to the small size of the pretraining corpus used in our experiments:
%\citet{hu20icml} report low correlation between \abr{pos} tagging accuracy and the pretraining corpus size.
%However,  \citet{lauscher2020zero} show that the pretraining corpus size is one of the top correlated feature for \abr{nli}.

\begin{figure}[th]
    \centering
    \includegraphics[width=0.45\textwidth]{\figfile{pos_150K_continued_accuracy}}
    \caption{
    %TODO: update with new figure for ta and vi
    \abr{pos} tagging accuracy after continued training on the Bible of each target language.
    The continued training gives surprising improvement in the model pretrained on multiple languages.
    }
    \label{fig:pos_unseen_continued_el}
\end{figure}


\begin{figure}[th]
    \centering
    \includegraphics[width=0.45\textwidth]{\figfile{ner_150K_continued_f1}}
    \caption{
    %TODO: update with new figure for ta and vi
    \abr{ner} F1 scores after continued training on the Bible of each target language.
    %, using the five different pretrained models as an initialized model.
    The continued training gives limited improvement in most languages on \abr{ner} when compared to \abr{pos} tagging.
    % surprising improvement in the model pretrained only using English, performing on par with multilingual models.
    }
    \label{fig:ner_unseen_continued}
\end{figure}


\subsection{Findings for RQ3}

%\begin{table}[t]
%\centering
%\small
%\setlength{\tabcolsep}{7pt}
%\begin{tabular}{lrrrr}
%\toprule
%\textbf{Pretrain Lang} & \textsc{en} & \textsc{de} & \textsc{nl} & \textbf{Unseen}  \\
%% Add indivdiual columns for each 5 language.
%\midrule
%\textsc{en}             & .951 & .245 & .311 & .193 \\
%Rel-2 (+de)              & .949 & .791 & .328 & .192 \\
%Rel-3 (+sv)              & .951 & .799 & .392 & .223 \\
%Rel-4 (+nl)              & .949 & .800 & .865 & .225 \\
%Rel-5 (+da)              & .949 & .813 & .874 & .237 \\
%\bottomrule
%\end{tabular}
%\caption{\label{tab:pos_unseen_related}
%\abr{pos} tagging accuracy after pretraining on a set of up to 5 related languages and finetuning on English.
%}
%\end{table}
%%TODO: Confrim the results with different random starts/seeds

\begin{table*}[th]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|rr|rrrrrrrrrrrrr}
\toprule
\textbf{Pretrain} & en & de   & ru  & zh    & ar   & hi   & bg  & el   & es   & fr   & sw   & th   & tr   & ur   & vi   \\
\midrule                                                           
\textsc{en}   & .731        & .375 & .343 & .340 & .339 & .345 & .347 & .346 & .404 & .381 & .366 & .350 & .358 & .347 & .354 \\
Rel-2         & .733 & .536 & .363 & .350 & .357 & .361 & .359 & .367 & .422 & .384 & .374 & .360 & .381 & .363 & .369 \\
Rel-3         & .721        & .535 & .351 & .349 & .350 & .355 & .350 & .352 & .434 & .420 & .383 & .357 & .382 & .348 & .370 \\
Rel-4         & .710        & .493 & .350 & .336 & .348 & .355 & .354 & .349 & .433 & .409 & .368 & .360 & .373 & .347 & .363 \\
Rel-5         & .726        & .527 & .339 & .335 & .335 & .342 & .343 & .342 & .430 & .415 & .376 & .339 & .372 & .335 & .347 \\
\bottomrule
\end{tabular}
\caption{\label{tab:xnli_related}
\abr{nli} accuracy on the 13 unseen languages using the models pretrained on related languages (\textsc{en, de, sv, nl, da}), incrementally added one language at a time up to five languages.
}
\end{table*}

\begin{figure}[th]
    \centering
    \includegraphics[width=0.49\textwidth]{\figfile{related_pos_150K}}
    \caption{\abr{pos} tagging accuracy using related pretraining languages (\textsc{en, de, sv, nl, da}) grouped by families of target languages, with Indo-European (\abr{ie}) languages further divided into subgroups following the \abr{xtreme} dataset.
    The change in accuracy is mainly in Germanic, Romance, and Uralic languages due to only using pretraining languages from Germanic family. 
    %\jbgcomment{why?}
    }
    \label{fig:pos_unseen_related}
\end{figure}


\paragraph{POS Tagging}
%Results on models pretrained on related languages slightly different trend in terms of cross-lingual transfer across language families.
%Results on models pretrained on related languages shows a different trend in terms of cross-lingual transfer across language families.
%Figure~\ref{fig:pos_unseen_related} shows the zero-shot \abr{pos} tagging results for models pretrained on related languages.
In contrast to \abr{rq}1, \abr{pos} tagging accuracy for most languages does not change much when increasing the number of pretraining languages (Figure~\ref{fig:pos_unseen_related}). 
The unseen languages on which we observe gains 
%from  adding more related pretraining languages 
belong to the Germanic (\textsc{af}, \textsc{nl}), Romance (\textsc{es}, \textsc{it}, \textsc{fr}, \textsc{pt}), and Uralic (\textsc{et}, \textsc{fi}, \textsc{hu}) language families. Those languages are spoken in Europe and relatively (as compared to the other language families) close to English.
The accuracy on languages from other language families changes by $<10\%$, which is smaller than the change for a diverse set of pretraining languages.
This indicates that the models pretrained on similar languages struggle to transferring to unrelated languages. 
%Using dissimilar pretraining languages is thus important for a wide applicability of the resulting models.
%However, still the trend of ``more languages the better for unseen languages'' holds for the models pretrained on related languages shown by the improved average POS tagging accuracy in Table~\ref{tab:pos_unseen_related}.


\paragraph{NER}
%Figure~\ref{fig:ner_unseen_related_avg} shows the results on the \abr{ner} task.
F1 scores of \abr{en}, Rel-2, Rel-3, Rel-4, and Rel-5 are .218, .219, .227, .236, and .237 respectively. 
Compared to Div-X, pretraining on related languages also improves up to adding five languages, however, those models brings relatively less improvement, similar to the \abr{pos} tagging.

\paragraph{NLI} Table \ref{tab:xnli_related} shows a similar trend for \abr{nli}: when adding related pretraining languages, accuracy on languages far from English either does not change much or decreases. In fact, for nine out of thirteen unseen target languages, Rel-5 is the worst.

%the trend of ``more languages the better for unseen languages'' is also observed in the NLI task using models pretrained on related languages.
%However, the differences in the NLI accuracy across the models using different number of pretraining languages are relatively small (within 5 percent points). 
%This results further indicate that the NLI results can be further explored better with larger size of the pretraining corpora.
%Overall, the ``curse of multilinguality'' is less of an issue for unseen languages up to five languages.
%It's relatively more of an issue than pretraining on diverse language sets than on pretraining using related languages.


% optional?
%\subsection{Pretraining on a Larger Corpus}
%Finally, we confirm whether the results change depending on the corpus size.



==> 2021_emnlp_multilingual_zeroshot/old_sections/60-analysis-back.tex <==


%\section{Analysis on the Effect of Limitations in Prior Experiments}
%\section{Experiments in Real World Setting: On Low-Resource Languages}
\section{More Pretraining Languages and Applying to Low-Resource Languages}
%\section{Comparison with \abr{xlm}}
\label{sec:xlmr}
%\section{Scalability of Adaptation on Models Pretrained on More Languages}

Our main takeaways from the last section are: 
(\abr{rq}1) without model adaptation, increasing pretraining languages does not improve accuracy on unrelated unseen target languages;
(\abr{rq}2) model adaptation largely helps exploiting models pretrained on more languages; and 
(\abr{rq}3) if using more than one pretraining language, diversity is important.

However, there are limitations in the experiment settings in Section~\ref{sec:results}.
We assume the following:
(1) relatively small pretraining corpora; 
(2) the target languages are included when building the model's vocabulary;
(3) fixed computational resources; and 
(4) pretraining languages up to 10. 
We now explore if our findings in \abr{rq}1 and \abr{rq}2 hold without such limitations.
For this, we use two publicly available pretrained \abr{\abr{xlm}} models \citep{conneau2019xlm}, which have been pretrained on full size Wikipedia in 17 (\abr{xlm}-17) and 100 (\abr{xlm}-100) languages, and \abr{xlm-r} base model trained on a larger Common Crawl corpus~\citep{conneau2020xlmr}.
We conduct a case study on low-resource languages unseen for all  models, including unseen vocabularies: Maltese (\textsc{mt}), Wolof (\textsc{wo}), Yoruba (\textsc{yo}), Erzya (\textsc{myv}), and Northern Sami (\textsc{sme}).
All pretraining languages used in Div-X are included in \abr{xlm}-17 except for Finnish, and all 17 pretraining languages for \abr{xlm}-17 are a subset of the pretraining languages for \abr{xlm}-100.
We report the averages with standard deviations from three random seeds.

%\subsection{Beyond Five Pretraining Languages} 
%Figure~\ref{fig:pos_5morelangs_eachlang} shows the result beyond five pretraining languages, up to 10 languages.
%The findings from previous section do hold that addition of pretraining language improves only related languages (e.g., adding Spanish improves other Romance languages).
%%Addition of Spanish (Romance) and Finnish (Urlaic) due to 
%
%Next, we also look into the results on languages that are not seen when building vocabularies on pretraining languages beyond  five languages.

%We also further look into languages beyond 


%\begin{figure}[th]
%    \centering
%    \includegraphics[width=0.49\textwidth]{\figfile{5morelangs_pos_acc}}
%    \caption{
%    something
%    %\abr{pos} tagging accuracy on diverse pretraining languages (\textsc{en, ru, zh, ar, hi}) grouped by families of target languages, with Indo-European (\abr{ie}) languages further divided into subgroups following \abr{xtreme}.
%    %The accuracy gain is significant for seen pretraining languages, and also the languages from the same family of the pretraining languages when added. 
%    }
%    \label{fig:pos_5morelangs}
%\end{figure}

% \begin{figure*}[th]
%     \centering
%     \includegraphics[width=0.99\textwidth]{\figfile{pos_150K_beyond5_accuracy}}
%     \caption{
%     POS tagging accuracy on each language.
%     The accuracy gain is significant for seen pretraining languages, and also the languages from the same family of the pretraining languages when added. 
%     }
%     \label{fig:pos_5morelangs_eachlang}
% \end{figure*}


% TODO: Each language
% Average results

\begin{table*}[t]
\centering
%\setlength{\tabcolsep}{7pt}
\small
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Model} & \# lgs  & \textsc{mt} & \textsc{wo} & \textsc{yo} & \textsc{myv} & \textsc{sme}\\
\midrule
\multicolumn{4}{l}{\bf Before Model Adaptation} \\
% Add indivdiual columns f.
% Diverse-2   & 2         172 & .447 \\
% Div-2 (+ru)       & 2    &.135 & .200 & .172 & $.442 \pm .007$ & .174\\
% Div-5 (+hi)       & 5    &.162 & .215 & .186 & .437       & .202 \\
Div-5 (+hi)       & 5    &$.159 \pm .019$ & $.214 \pm .029$ & $.183 \pm .012$ & $.419 \pm .016$  & $.200 \pm .012$ \\
Div-6  (+es)      & 6    & $.196 \pm .021$ &  $.256 \pm .020$ & $.183 \pm .004$ & $.437 \pm .010$ & $.249 \pm .001$\\
%Div-7 (+el)       & 7    & $.165 \pm .015$ & $.225 \pm .031$ & $.182 \pm .013$ & $.404 \pm .006$ & $.225 \pm .024$\\
Div-8 (+fi)       & 8    & $.176 \pm .002$ & $.236 \pm .013$ & $.178 \pm .001$ & $.435 \pm .025$ & $.320 \pm .023$ \\
Div-10 (+tr)      & 10   & $.171 \pm .004$ & $.243 \pm .016$ & $.184 \pm .007$ & $.420 \pm .008$ & $.315 \pm .013$ \\
\abr{xlm}-17      &17    & $.214\pm .007 $  & $.276 \pm .009$ & $.247 \pm .033$    & $.436\pm .035$      & $.318 \pm .010$ \\
\abr{xlm}-100     &100   & $.233 \pm .017$ & $.280 \pm .019$ & $.231 \pm .026$ & $.434 \pm .027$ & $.351 \pm .026$ \\
\abr{xlm-r}       & 100  &$.221 \pm .033$     & $.260 \pm .030$     & $.263 \pm .034$   & $.490 \pm .022$ & $.344 \pm .052$      \\
\midrule                             
\multicolumn{4}{l}{\bf After Model Adaptation} \\


Div-5 (+hi)   & 5         & $.272 \pm {.007}$ & $.388\pm{.018}$ & $.251\pm{.025}$ & $.489\pm{.013}$ & $.361\pm{.051}$ \\
Div-6 (+es)   & 6         & $.310 \pm .007$ & $.366 \pm .010$ & $.253 \pm .008$ & $.492 \pm .012$ & $.377 \pm .005$\\
Div-8 (+fi)   & 8         & $.315 \pm .002$ & $.384 \pm .036$ & $.257 \pm .017$  & $.527 \pm .016$        & $.449 \pm .005$ \\
Div-10 (+tr)  & 10        & $.298 \pm .044$ & $.389 \pm .059$ & $.251 \pm .004$ & $.508 \pm .040$ & $.457 \pm .005$ \\
\abr{xlm}-17  & 17        & $.451 \pm .002$ & $.410 \pm .047$ & $.361 \pm .032$ & $.603 \pm .011$ & $.567 \pm .042$ \\
\abr{xlm}-100 & 100       & $.627 \pm .026$ & $.673 \pm .015$ & $.385 \pm .071$ & $.697 \pm .015$ & $.752 \pm .006$ \\
\abr{xlm-r}   & 100       & $.594 \pm .010$ & $.689 \pm .005$ & $.509 \pm .008$ & $.720 \pm .007$ & $.703 \pm .007$   \\
\bottomrule
\end{tabular}
\caption{\label{tab:pos_scale}
\abr{pos} tagging accuracy of our models pretrained on diverse languages, \abr{xlm}-17, \abr{xlm}-100, and \abr{xlm-r} after finetuning on English.
The models before adaptation are roughly on par regardless of the number of pretraining languages, and the models after adaptation is more affected by the related pretraining languages. 
%The \abr{xlm}-R results reported in this table is not the publicly available pretrained one and rather the one we trained on a downsampled data with smaller number of pretraining languages.
}
%\jbgcomment{Needs takeaway}
\end{table*}


\subsection{Results} 
%\subsection{Results on Languages not Included when Building Vocabulary} 
%\jbgcomment{perform is vague}


\paragraph{RQ1} 
For models without adaptation,
accuracy does not improve for increasing numbers of source languages (Table~\ref{tab:pos_scale}). 
Indeed, the accuracy on both \abr{xlm}-17 and \abr{xlm}-100 are on par even though the former uses 17 pretraining languages and the latter uses 100. 
One exception is on Northern Sami (Uralic language with Latin script)
due to \abr{xlm}-17 not seeing any Uralic languages, but \abr{xlm}-100 does during pretraining.
%Indeed, with $43.7\%$, Diverse-5 even achieves higher accuracy both \abr{xlm}-17 and \abr{xlm}-100 on Erzya, which obtain an accuracy of $33.8\%$ and $31.2\%$, respectively. 
%Additionally, \abr{xlm}-17 performs better than \abr{xlm}-100 on two of the remaining three languages. 
%This confirms our finding that adding more than four pretraining languages does not result in performance gains on unseen and unrelated target languages.

When further comparing Div-10 and \abr{xlm}-17, addition of pretraining languages help for Maltese and Yoruba.
Addition of Spanish even improved accuracy outside Romance languages, such as Maltese (Afro-Asiatic), and Wolof (Niger-Congo).
Erzya remains constant from five to 100 languages, even increasing the pretraining corpus size from downsampled (Div-X) to full Wikipedia (\abr{xlm}-17 and \abr{xlm}-100), suggesting that the transfer across language families are primarily happening in languages written in Latin scripts.
The pretraining corpus size is not an issue for \abr{pos} tagging since Div-X models have comparable accuracy to \abr{xlm}-17 and \abr{xlm}-100 without the model adaptation.


\paragraph{RQ2} 
For the models with adaptation,
there is a significant gap between \abr{xlm}-17 and \abr{xlm}-100.
%In Maltese and Wolof, the accuracy differences are significant, which are further confirmed by obtaining results using multiple random seeds.
This confirms our findings in the last section: more pretraining languages may be beneficial. 
%However, those results are limited to \emph{unrelated} target languages. 
Thus, a possible explanation is that one or more of \abr{xlm}-100's pretraining languages is similar to our target languages and such languages can only be exploited through continued pretraining.
Therefore, having the model see more languages during pretraining is better when the models can be adapted to each target language.

%This hypothesis is further backed up by Diverse-5, as predicted by the experiments in the last section, outperforming \abr{xlm}-17 on two of the four languages, even though it has fewer pretraining languages than \abr{xlm}-17. 

%Assuming we have a small portion of a monolingual corpus available in the target language such as the Bible, 
%more languages helps for continued pretraining.
%Largely relying on the related languages.
%In contrast to \citet{artetxe2020crosslingual}, where they conduct model adaptation from the pretrained English model using the full-size Wikipedia in each target language, model adaptation using the Bible requires closely related languages in the pretrained languages.

%However, surprisingly small portion of the languages and data are needed to extend in a comparable manner to \abr{xlm}-100, the massive multilingual model trained on full corpus of 100 Wikipedia datasets.





==> 2021_emnlp_multilingual_zeroshot/old_sections_aclrr_nov/10-intro.tex <==
\section{Introduction}

% Widely used pretrained LMs
Pretrained multilingual language models \cite{devlin2019bert,conneau2020xlmr} are now a standard approach for cross-lingual transfer in natural language processing (\abr{nlp}).
However, there are multiple, potentially related issues on pretraining multilingual models.
\citet{conneau2020xlmr} find ``curse of multilinguality'': 
for a fixed model size, zero-shot performance on target languages seen during pretraining increases with additional pretraining languages only until a certain point, after which performance decreases.
%In other words, there is a trade-off between cross-lingual transfer to low-resource languages and the overall transfer on high- and low-resource languages.
\citet{wang2020negative} also report ``negative interference'', where monolingual models achieve better results than multilingual models, both on subset of high- and low-resource languages.
However, those findings are limited to target languages seen during pretraining.

Current multilingual models cover only a small subset of the world's languages. Furthermore, due to data sparsity, monolingual pretrained models are not likely to obtain good results for many low-resource languages. In those cases, multilingual models can  zero-shot learn for unseen languages with an above-chance performance, which can be further improved via model adaptation of target-language text~\citep{wang2020extending} even with limited amounts~\citep{ebrahimi2021adapt}. However, it is poorly understood how the number of pretraining languages influences performance in those cases.
Does the ``curse of multilinguality'' or the ``negative interference'' also negatively impact performance on %target languages unseen during pretraining? 
unseen target languages?
And, if we want a model to be applicable to as many unseen languages as possible, how many languages should it be trained on?

% Introduce EXACT research questions (1, 2, and 3)
% The more intro., the better for JBG

%Some languages do not have enough texts to be included during the pre-training

% TODO: Why would you look at languages not seen? Why not focus on adapted models?
%However, 

%extinct, dialect, no written corpus exits


%the popular pretrained models such as mBERT and XLM-R, and analysis during the pretraining process is limited.
%Furthermore, some work CITEME did not use such popular pretrained models and conducted further analysis, but still analysis on the effect towards unseen languages during pre-training is limited.

Specifically, we ask the following research questions: 
(1) How does pretraining on an increasing number of languages impact zero-shot performance on unseen target languages?
(2) Does the effect of the number of pretraining languages change with model adaptation to target languages?
%(3) Do the results of the aforementioned RQs change 
(3) Does the answer to the first research question change if the pretraining languages are all related to each other? 
%Given that pretraining multilingual models have 
%we assume that the computational resources are limited throughout this paper, also limiting the number of pretraining languages to explore. 
%Training steps, model size, number of pretraining languages.

% ``small world'' constraint
%One problem of pretraining multilingual models from scratch is its intense computational cost.
%To be more realistic for practitioners to pretrain a model from scratch considering the computational cost, we further assume computational resources are limited throughout experiments we conduct in this paper.
%Given the computational constraints, we seek to find the best strategies to pretrain a multilingual model by focusing on the number of pretraining languages.
%We ask the following research questions: 
%(1) Does pretraining on more languages improve zero-shot performance on unseen languages?
%(2) Does the effect of the number of pretraining languages change with model adaptation to target languages?
%(3) Do the results of the aforementioned RQs change if the pretraining languages are all related to each other? 

%This paper analyzes multilingual pretrained models trained on up to five source languages on two zero-shot cross-lingual downstream tasks on unseen languages: part-of-speech (\abr{pos}) tagging and natural language inference (\abr{nli}).
%We further continue pretraining on the pretrained multilingual models on target languages: results are consistent and mostly independent of pretraining languages.
%Multilingual training  generally improves zero-shot cross-lingual transfer for unseen languages, however, diminishing returns set in compared to adding related languages. 
We pretrain a variety of monolingual and multilingual models, which we then finetune on English and apply to three zero-shot cross-lingual downstream tasks in unseen target languages: part-of-speech (\abr{pos}) tagging, named entity recognition (\abr{ner}), and natural language inference (\abr{nli}).
%Such settings include 
%(1) multilingual models pretrained on diverse pretraining languages from multiple language families,
%(2) models further continued pretraining on the target languages, and 
%(3) models pretrained on languages that are related to each other.
%Our results show that the improvement from adding more pretraining languages on plateaus at approximately 4. However, its accuracy after continued pretraining is on par between one pretraining language and multiple pretraining languages.
Experimental results suggest that choosing a diverse set of pretraining languages is crucial for effective transfer.
Without model adaptation, increasing the number of pretraining languages improves accuracy on unrelated unseen target languages at first and plateaus thereafter. 
Last, with model adaptation, additional pretraining languages beyond English generally help. 

We are aware of the intense computational cost of pretraining and its environmental impact~\citep{strubell2019energy}. Thus,
we opt to perform our experiments in Section~\ref{sec:results} on a relatively small scale with a fixed computational budget for each model, but validate our most central findings in Section~\ref{sec:xlmr} on large pretrained models which are already publicly available. 

%\jbgcomment{``pairwise'' related language is unclear, so I removed}



%%---------removed paragraphs------------%%

%Our contributions are as the followings: (1) Adding more languages helps for unseen languages up to a certain limit. Unless the target languages are related to one of the pre-training languages, and (2) (FIXME) the results on unseen languages are consistent even after employing model adaption by continued pre-training on target languages.

%Our contributions are as the followings: (1) Adding more languages helps for unseen languages up to a certain limit. Unless the target languages are related to one of the pre-training languages, and (2) (FIXME) the results on unseen languages are consistent even after employing model adaption by continued pre-training on target languages.


%The number of pre-training languages, shown to have on natural language inference task.

%We evaluate pretrained models on multiple checkpoints while pretraining, showing that the optimal performance on unseen languages is achieved at the early stage of pretraining.

% \begin{itemize*}
%  \item Adding more languages helps for unseen languages up to a certain limit. Unless the target languages are related to one of the pre-training languages
%  \item The more languages the better after doing model adaption by continued pre-training on target languages. 
 %\item We show that overly pretraining on source languages can hinder cross-lingual transfer to unseen languages during pretraining. Early stopping during pretraining is important when transferring to unseen languages.
 %\item We show that unseen languages which are typologically distant from the pretraining languages are moderately affected.
 %\item We show that the more languages the better up to five pre-training languages.
 %\item Convergence is slower for more and diverse languages
 %\item Harder for the NLI task than syntactic tasks.
% \end{itemize*}

%Cautious about the segmented and unsegmented languages. Encouraging Chinese and Japanese to be separately learned during pre-training.

%Sufficient amount of written texts in all domain and language does not exist.

%{\bf Research Question 1:} Does adding a diverse set of languages during pre-training help or hurt languages unseen during pre-training in downstream tasks?

%Diverse languages = languages distant from English


==> 2021_emnlp_multilingual_zeroshot/old_sections_aclrr_nov/20-background.tex <==
\section{Cross-lingual Transfer via Pretraining}

Pretrained multilingual models are a straightforward cross-lingual transfer approach: a model pretrained on multiple languages is then fine-tuned on target-task data in the \emph{source} language. Subsequently, the model is applied to target-task data in the \emph{target} language. Most commonly, the target language is part of the model's pretraining data. However, cross-lingual transfer is possible even if this is not the case, though performance tends to be lower. This paper extends prior work exploring the cross-lingual transfer abilities of pretrained models for \emph{seen} target languages depending on the number of pretraining languages to \emph{unseen} target languages.
We now transfer via pretrained multilingual models and introduce the models and methods vetted in our experiments.

\subsection{Background and Methods}
\paragraph{Pretrained Language Models}
Contextual representations such as ELMo~\citep{peters2018elmo} and \bert{}~\citep{devlin2019bert} are not just useful for monolingual representations.  Multilingual \bert{}~\citep[\mbert{}]{devlin2019bert}, \abr{xlm}~\citep{conneau2019xlm}, and XLM-RoBERTa~\citep[\abr{xlm-r}]{conneau2020xlmr} have surprisingly high cross-lingual transfer performance compared to the previous best practice: static cross-lingual word embeddings~\citep{pires2019multilingual,wu2019beto}.
Multilingual models are also practical---why have hundreds of separate models for each language when you could do better with just one?
Furthermore, \citet{wu2020languages} reports that models pretrained on 100+ languages is better than bilingual or monolingual language models in zero-shot cross-lingual transfer.
%However, there's a catch. 
%\citet{conneau2020xlmr} reports the ``curse of multilinguality'': as the number of pretraining languages increases, the better the cross-lingual transfer is up to some point, after which the performance in zero-shot transfer starts to decrease.
%Our work complements \citet{conneau2020xlmr} by explicitly dividing up between seen and unseen languages during pretraining and testing whether the ``curse of multilinguality'' is also an issue for unseen languages too.

\paragraph{Model Adaptation to Unseen Languages}
Adapting pretrained multilingual models, such as \mbert{} and \abr{xlm-r}, to unseen languages is one way to use such models beyond the languages covered during pretraining time.
%and therefore, adapting to languages unseen during the pretraining step is a common approach.
%, and the rest of languages are not seen during the pretraining step.
%A common practice is for to use multilingual language model for languages unseen at the pretraining time is to conduct model adaptation. \jbgcomment{do not understand previous sentence}
Several methods for adapting pretrained multilingual language models to unseen languages have been proposed in the literature, including continuing masked language model (\abr{mlm}) training~\citep{chau2020parsing,muller2020when} optionally adding Adapter 
%\jbgcomment{Not adaptor?}
%\yfcomment{Not adaptor, I checked the original paper too -- KK: agreed}
modules~\citep{pfeiffer2020mad}, or extending the vocabulary of the pretrained models~\citep{artetxe2020crosslingual,wang2020extending}. 
%Later work shows that continued pretraining by \abr{mlm} is effective method for adapting pretrained models CITE\_ABTEEN.
However, such adaptation methods assume the existence of sufficient monolingual corpora in the target languages.
Some spoken languages, dialects, or extinct languages lack monolingual corpora to conduct model adaptation, which motivates us to look into the performance of languages unseen during pretraining.

\jbgcomment{previous paragraph is a little disjointed, consider rewriting with a clear topic sentence}

\subsection{Research Questions}
A single pretrained model that can be applied to any language, including those unseen during pretraining, is both more efficient and more practical than pretraining one model per language. 
%Moreover, it is the \emph{only option} for unknown target languages or for languages without enough resources for pretraining.
Moreover, it is the only practical option for unknown target languages or for languages without enough resources for pretraining.
Thus, models that can be applied or at least easily adapted to unseen languages are an important research focus. This work addresses the following research questions (\abr{rq}), using English as the source language for finetuning.

% RQ1: The more languages the better?
\noindent\textit{{\bf RQ1}: How does the number of pretraining languages influence zero-shot performance on unseen target languages?}

%EXPLANATION HERE
We first explore how many languages a model should be pretrained on
if the target language is unknown at test time or has too limited monolingual resources for model adaptation.
On one hand, we hypothesize that increasing the number of pretraining languages will improve performance, as the model sees a more diverse set of scripts and linguistic phenomena. Also, the more pretraining languages, the better chance of having a related language to the target language.
%On the other hand, however, the ``curse of multilinguality'' could affect unseen target languages as well: other languages could distract from English, the finetuning source language, and, thus, lower performance.
However, multilingual training can cause interference:  other languages could distract from English, the finetuning source language, and thus, lower performance.

% RQ2: The more languages the better AFTER doing model adaption (continued MLM on the target language)?
\noindent\textit{{\bf RQ2}: How does the answer to RQ1 change with model adaptation to the target language?}

%EXPLANATION HERE
This question is concerned with settings in which we have enough monolingual data available to adapt a pretrained model to the target language.
Similar to our hypothesis for \abr{rq}1, we expect that having seen more pretraining languages should make adaptation to unseen target languages easier. However, another possibility is that the process of adapting the model makes any languages other than the finetuning source language unnecessary, such that performance stays the same or decreases when adding more pretraining languages. 

% RQ3: Do the results in RQ1 and RQ2 change, if we use related languages for pretraining?
\noindent\textit{{\bf RQ3}: Do the answers to \abr{rq}1 change if all pretraining languages are related to each other?}

%EXPLANATION HERE
We use a diverse set of pretraining languages when exploring \abr{rq}1, since we expect that to be maximally beneficial. 
However, the results might change depending on the exact languages.
%, especially when a different set of pretraining languages is used.
Thus, as a case study, we repeat all experiments
using a set of closely related languages.
On the one hand, we hypothesize that benefits due to adding more pretraining languages (if any) will be smaller with related languages, as we reduce the diversity of linguistic phenomena in the pretraining data. However, on the other hand, if English is all we use during fine-tuning, performance might increase with related languages, as this will approximate training on more English data more closely.


==> 2021_emnlp_multilingual_zeroshot/old_sections_aclrr_nov/70-related_work.tex <==
\section{Related Work}

\paragraph{Static Cross-Lingual Word Embeddings}
Static cross-lingual word embeddings \citep{mikolov2013exploit,lample2018word} embed and align words from multiple languages for downstream \abr{nlp} tasks~\citep{lample2018unsupervised,D18-1398}.
%However, since prior work~\citep{ahmad2019cross,artetxe2020crosslingual} report that pretrained multilingual language models are superior on languages seen during pretraining, most work has transitioned from static cross-lingual word embeddings to multilingual language models.
\citet{lin2019choosing} explore the selection of transfer language using both data-independent (e.g., typological) features, and data-dependent features (e.g., lexical overlap). 
Static cross-lingualare often supervised with bilingual lexicon
Their work is on static cross-lingual word embeddings, whereas, this paper explores the effect on pretrained language models.

\jbgcomment{I think you can talk more in depth about word embeddings: contrast the supervision of the approaches and compare the massively multilingual word embeddings}

\yfcomment{TODO: Mention that Bilingual lexicons are needed for supervised cross-lingual word embeddings, pretrained models are closer to unsupervised cross-lingual word embeddings}

\paragraph{Analysis of Pretrained Multilingual Models on Seen Languages}
Starting from  \citet{pires2019multilingual}, analysis of the cross-lingual transferability of pretrained multilingual language models has been a topic of interest. 
\citet{pires2019multilingual} hypothesize that the cross-lingual transfer occurs due to shared tokens across languages, but  \citet{artetxe2020crosslingual} showed that cross-lingual transfer can be successful even among languages without shared scripts.
Other work %on pretrained multilingual language models 
investigated the relationship between zero-shot cross-lingual learning and typological features \citep{lauscher2020zero}, encoding language-specific features~\citep{libovicky2020language}, and %further in-depth analysis and improvement on 
\mbert{}'s multlinguality~\citep{dufter2020identifying}.
However, the majority of the analyses have either been limited to large public models (\mbert{} or \abr{xlm-r}) or to up to two pretraining  languages \citep{k2020crosslingual,wu2020languages}.
Here, we analyze the ability of models to benefit from an increasing number of pretraining languages.

\jbgcomment{Can you connect this related work more to what you've done?}

%\paragraph{Adapting to Unseen Languages}
%One issue for the widely used mBERT and XLM-R is that those models cover around 100 languages during pretraining.
%One common practice to use multilingual language model for languages unseen at the pretraining time is to conduct model adaptation. 
%Several of such adaptation methods for pretrained multilingual language models to unseen languages has been proposed in the literature, including continuing masked language model (MLM) training~\citep{chau-etal-2020-parsing,muller2020when} optionally adding Adapter modules~\citep{pfeiffer-etal-2020-mad}, or extending the vocabulary of the pretrained models~\citep{artetxe2020crosslingual,wang-etal-2020-extending}. 
%Later work shows that continued pretraining by MLM to be the effective method for adapting pretrained models CITE\_ABTEEN.
%However, such adaptation method assumes the existence of monolingual corpus in the target languages.
%Some spoken languages, dialects, or extinct languages lack monolingual corpus to conduct model adaptation, which motivates us to look into the performance of languages unseen during pretraining.



==> 2021_emnlp_multilingual_zeroshot/old_sections_aclrr_nov/80-conclusion.tex <==
\section{Conclusion}
% What is done
This paper explores pretraining on different numbers of languages has on unseen target languages after finetuning on English:
(1) without model adaptation, improvement by pretraining on more languages is limited as we add more languages; 
(3) when pretraining on more than one language, choosing a diverse set is important. 

Future directions include analyzing the effect of multilingual pretraining from different perspectives such as different pretraining tasks and architectures, e.g., mT5~\citep{xue2021mt5}, and more complex tasks beyond classification or sequence tagging.

\jbgcomment{Is it possible to make these suggestions firmer?  E.g., tell people how many languages you need, what constitutes diversity, etc.?  If we want this paper to get cited, we need a rulebook that people should follow for multilingual LMs.}

\yfcomment{Should be based on the regression analysis.}

% We further validate our findings using XLM-17 and XLM-100, two publicly available models pretrained on 17 and, respectively, 100 languages.


%Therefore, we suggest to open up opportunities for using English-only models as an initial model to continue pretraining when adapting to languages unseen during pretraining.
%Finally, we confirmed that the pretraining languages that are related to each other further improves on unseen languages as the number of pretraining languages increases up to five.


%One of the limitations of analysis and experiments conducted in this paper is the models pretrained on small scale corpora, which can make large difference especially on the NLI task.
%Future work remains on analyzing and exploring models large scale pretraining corpora, and furthermore experimenting on pretraining corpora other than Wikipedia.
